Deinterleaving RADAR emitters with optimal transport distances

Detection and identification of emitters provide vital information for defensive strategies in electronic intelligence. Based on a received signal containing pulses from an unknown number of emitters, this paper introduces an unsupervised methodology for deinterleaving RADAR signals based on a combination of clustering algorithms and optimal transport distances. The first step involves separating the pulses with a clustering algorithm under the constraint that the pulses of two different emitters cannot belong to the same cluster. Then, as the emitters exhibit complex behavior and can be represented by several clusters, we propose a hierarchical clustering algorithm based on an optimal transport distance to merge these clusters. A variant is also developed, capable of handling more complex signals. Finally, the proposed methodology is evaluated on simulated data provided through a realistic simulator. Results show that the proposed methods are capable of deinterleaving complex RADAR signals.

==> divers/divers.tex <==
% *** GRAPHICS RELATED PACKAGES ***
%
\ifCLASSINFOpdf
  % \usepackage[pdftex]{graphicx}
  % declare the path(s) where your graphic files are
  % \graphicspath{{../pdf/}{../jpeg/}}
  % and their extensions so you won't have to specify these with
  % every instance of \includegraphics
  % \DeclareGraphicsExtensions{.pdf,.jpeg,.png}
\else
  % or other class option (dvipsone, dvipdf, if not using dvips). graphicx
  % will default to the driver specified in the system graphics.cfg if no
  % driver is specified.
  % \usepackage[dvips]{graphicx}
  % declare the path(s) where your graphic files are
  % \graphicspath{{../eps/}}
  % and their extensions so you won't have to specify these with
  % every instance of \includegraphics
  % \DeclareGraphicsExtensions{.eps}
\fi
% graphicx was written by David Carlisle and Sebastian Rahtz. It is
% required if you want graphics, photos, etc. graphicx.sty is already
% installed on most LaTeX systems. The latest version and documentation
% can be obtained at: 
% http://www.ctan.org/pkg/graphicx
% Another good source of documentation is "Using Imported Graphics in
% LaTeX2e" by Keith Reckdahl which can be found at:
% http://www.ctan.org/pkg/epslatex
%
% latex, and pdflatex in dvi mode, support graphics in encapsulated
% postscript (.eps) format. pdflatex in pdf mode supports graphics
% in .pdf, .jpeg, .png and .mps (metapost) formats. Users should ensure
% that all non-photo figures use a vector format (.eps, .pdf, .mps) and
% not a bitmapped formats (.jpeg, .png). The IEEE frowns on bitmapped formats
% which can result in "jaggedy"/blurry rendering of lines and letters as
% well as large increases in file sizes.
%
% You can find documentation about the pdfTeX application at:
% http://www.tug.org/applications/pdftex




% *** MATH PACKAGES ***
%
%\usepackage{amsmath}
% A popular package from the American Mathematical Society that provides
% many useful and powerful commands for dealing with mathematics.
%
% Note that the amsmath package sets \interdisplaylinepenalty to 10000
% thus preventing page breaks from occurring within multiline equations. Use:
%\interdisplaylinepenalty=2500
% after loading amsmath to restore such page breaks as IEEEtran.cls normally
% does. amsmath.sty is already installed on most LaTeX systems. The latest
% version and documentation can be obtained at:
% http://www.ctan.org/pkg/amsmath





% *** SPECIALIZED LIST PACKAGES ***
%
%\usepackage{algorithmic}
% algorithmic.sty was written by Peter Williams and Rogerio Brito.
% This package provides an algorithmic environment fo describing algorithms.
% You can use the algorithmic environment in-text or within a figure
% environment to provide for a floating algorithm. Do NOT use the algorithm
% floating environment provided by algorithm.sty (by the same authors) or
% algorithm2e.sty (by Christophe Fiorio) as the IEEE does not use dedicated
% algorithm float types and packages that provide these will not provide
% correct IEEE style captions. The latest version and documentation of
% algorithmic.sty can be obtained at:
% http://www.ctan.org/pkg/algorithms
% Also of interest may be the (relatively newer and more customizable)
% algorithmicx.sty package by Szasz Janos:
% http://www.ctan.org/pkg/algorithmicx




% *** ALIGNMENT PACKAGES ***
%
%\usepackage{array}
% Frank Mittelbach's and David Carlisle's array.sty patches and improves
% the standard LaTeX2e array and tabular environments to provide better
% appearance and additional user controls. As the default LaTeX2e table
% generation code is lacking to the point of almost being broken with
% respect to the quality of the end results, all users are strongly
% advised to use an enhanced (at the very least that provided by array.sty)
% set of table tools. array.sty is already installed on most systems. The
% latest version and documentation can be obtained at:
% http://www.ctan.org/pkg/array


% IEEEtran contains the IEEEeqnarray family of commands that can be used to
% generate multiline equations as well as matrices, tables, etc., of high
% quality.




% *** SUBFIGURE PACKAGES ***
%\ifCLASSOPTIONcompsoc
%  \usepackage[caption=false,font=normalsize,labelfont=sf,textfont=sf]{subfig}
%\else
%  \usepackage[caption=false,font=footnotesize]{subfig}
%\fi
% subfig.sty, written by Steven Douglas Cochran, is the modern replacement
% for subfigure.sty, the latter of which is no longer maintained and is
% incompatible with some LaTeX packages including fixltx2e. However,
% subfig.sty requires and automatically loads Axel Sommerfeldt's caption.sty
% which will override IEEEtran.cls' handling of captions and this will result
% in non-IEEE style figure/table captions. To prevent this problem, be sure
% and invoke subfig.sty's "caption=false" package option (available since
% subfig.sty version 1.3, 2005/06/28) as this is will preserve IEEEtran.cls
% handling of captions.
% Note that the Computer Society format requires a larger sans serif font
% than the serif footnote size font used in traditional IEEE formatting
% and thus the need to invoke different subfig.sty package options depending
% on whether compsoc mode has been enabled.
%
% The latest version and documentation of subfig.sty can be obtained at:
% http://www.ctan.org/pkg/subfig



% *** FLOAT PACKAGES ***
%
%\usepackage{fixltx2e}
% fixltx2e, the successor to the earlier fix2col.sty, was written by
% Frank Mittelbach and David Carlisle. This package corrects a few problems
% in the LaTeX2e kernel, the most notable of which is that in current
% LaTeX2e releases, the ordering of single and double column floats is not
% guaranteed to be preserved. Thus, an unpatched LaTeX2e can allow a
% single column figure to be placed prior to an earlier double column
% figure.
% Be aware that LaTeX2e kernels dated 2015 and later have fixltx2e.sty's
% corrections already built into the system in which case a warning will
% be issued if an attempt is made to load fixltx2e.sty as it is no longer
% needed.
% The latest version and documentation can be found at:
% http://www.ctan.org/pkg/fixltx2e


%\usepackage{stfloats}
% stfloats.sty was written by Sigitas Tolusis. This package gives LaTeX2e
% the ability to do double column floats at the bottom of the page as well
% as the top. (e.g., "\begin{figure*}[!b]" is not normally possible in
% LaTeX2e). It also provides a command:
%\fnbelowfloat
% to enable the placement of footnotes below bottom floats (the standard
% LaTeX2e kernel puts them above bottom floats). This is an invasive package
% which rewrites many portions of the LaTeX2e float routines. It may not work
% with other packages that modify the LaTeX2e float routines. The latest
% version and documentation can be obtained at:
% http://www.ctan.org/pkg/stfloats
% Do not use the stfloats baselinefloat ability as the IEEE does not allow
% \baselineskip to stretch. Authors submitting work to the IEEE should note
% that the IEEE rarely uses double column equations and that authors should try
% to avoid such use. Do not be tempted to use the cuted.sty or midfloat.sty
% packages (also by Sigitas Tolusis) as the IEEE does not format its papers in
% such ways.
% Do not attempt to use stfloats with fixltx2e as they are incompatible.
% Instead, use Morten Hogholm'a dblfloatfix which combines the features
% of both fixltx2e and stfloats:
%
% \usepackage{dblfloatfix}
% The latest version can be found at:
% http://www.ctan.org/pkg/dblfloatfix




%\ifCLASSOPTIONcaptionsoff
%  \usepackage[nomarkers]{endfloat}
% \let\MYoriglatexcaption\caption
% \renewcommand{\caption}[2][\relax]{\MYoriglatexcaption[#2]{#2}}
%\fi
% endfloat.sty was written by James Darrell McCauley, Jeff Goldberg and 
% Axel Sommerfeldt. This package may be useful when used in conjunction with 
% IEEEtran.cls'  captionsoff option. Some IEEE journals/societies require that
% submissions have lists of figures/tables at the end of the paper and that
% figures/tables without any captions are placed on a page by themselves at
% the end of the document. If needed, the draftcls IEEEtran class option or
% \CLASSINPUTbaselinestretch interface can be used to increase the line
% spacing as well. Be sure and use the nomarkers option of endfloat to
% prevent endfloat from "marking" where the figures would have been placed
% in the text. The two hack lines of code above are a slight modification of
% that suggested by in the endfloat docs (section 8.4.1) to ensure that
% the full captions always appear in the list of figures/tables - even if
% the user used the short optional argument of \caption[]{}.
% IEEE papers do not typically make use of \caption[]'s optional argument,
% so this should not be an issue. A similar trick can be used to disable
% captions of packages such as subfig.sty that lack options to turn off
% the subcaptions:
% For subfig.sty:
% \let\MYorigsubfloat\subfloat
% \renewcommand{\subfloat}[2][\relax]{\MYorigsubfloat[]{#2}}
% However, the above trick will not work if both optional arguments of
% the \subfloat command are used. Furthermore, there needs to be a
% description of each subfigure *somewhere* and endfloat does not add
% subfigure captions to its list of figures. Thus, the best approach is to
% avoid the use of subfigure captions (many IEEE journals avoid them anyway)
% and instead reference/explain all the subfigures within the main caption.
% The latest version of endfloat.sty and its documentation can obtained at:
% http://www.ctan.org/pkg/endfloat
%
% The IEEEtran \ifCLASSOPTIONcaptionsoff conditional can also be used
% later in the document, say, to conditionally put the References on a 
% page by themselves.




% *** PDF, URL AND HYPERLINK PACKAGES ***
%
%\usepackage{url}
% url.sty was written by Donald Arseneau. It provides better support for
% handling and breaking URLs. url.sty is already installed on most LaTeX
% systems. The latest version and documentation can be obtained at:
% http://www.ctan.org/pkg/url
% Basically, \url{my_url_here}.




% *** Do not adjust lengths that control margins, column widths, etc. ***
% *** Do not use packages that alter fonts (such as pslatex).         ***
% There should be no need to do such things with IEEEtran.cls V1.6 and later.
% (Unless specifically asked to do so by the journal or conference you plan
% to submit to, of course. )


% correct bad hyphenation here
\hyphenation{op-tical net-works semi-conduc-tor}




% if have a single appendix:
%\appendix[Proof of the Zonklar Equations]
% or
%\appendix  % for no appendix heading
% do not use \section anymore after \appendix, only \section*
% is possibly needed

% use appendices with more than one appendix
% then use \section to start each appendix
% you must declare a \section before using any
% \subsection or using \label (\appendices by itself
% starts a section numbered zero.)
%


\appendices
\section{Proof of the First Zonklar Equation}
Appendix one text goes here.

% you can choose not to have a title for an appendix
% if you want by leaving the argument blank
\section{}
Appendix two text goes here.


% use section* for acknowledgment
\section*{Acknowledgment}


The authors would like to thank...


% Can use something like this to put references on a page
% by themselves when using endfloat and the captionsoff option.
\ifCLASSOPTIONcaptionsoff
  \newpage
\fi



% trigger a \newpage just before the given reference
% number - used to balance the columns on the last page
% adjust value as needed - may need to be readjusted if
% the document is modified later
%\IEEEtriggeratref{8}
% The "triggered" command can be changed if desired:
%\IEEEtriggercmd{\enlargethispage{-5in}}

% references section

% can use a bibliography generated by BibTeX as a .bbl file
% BibTeX documentation can be easily obtained at:
% http://mirror.ctan.org/biblio/bibtex/contrib/doc/
% The IEEEtran BibTeX style support page is at:
% http://www.michaelshell.org/tex/ieeetran/bibtex/
%\bibliographystyle{IEEEtran}
% argument is your BibTeX string definitions and bibliography database(s)
%\bibliography{IEEEabrv,../bib/paper}
%
% <OR> manually copy in the resultant .bbl file
% set second argument of \begin to the number of references
% (used to reserve space for the reference number labels box)



\begin{thebibliography}{1}

\bibitem{IEEEhowto:kopka}
H.~Kopka and P.~W. Daly, \emph{A Guide to \LaTeX}, 3rd~ed.\hskip 1em plus
  0.5em minus 0.4em\relax Harlow, England: Addison-Wesley, 1999.

\end{thebibliography}

% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\begin{IEEEbiography}{Michael Shell}
Biography text here.
\end{IEEEbiography}

% if you will not have a photo at all:
\begin{IEEEbiographynophoto}{John Doe}
Biography text here.
\end{IEEEbiographynophoto}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

\begin{IEEEbiographynophoto}{Jane Doe}
Biography text here.
\end{IEEEbiographynophoto}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}



% that's all folks

% An example of a floating figure using the graphicx package.
% Note that \label must occur AFTER (or within) \caption.
% For figures, \caption should occur after the \includegraphics.
% Note that IEEEtran v1.7 and later has special internal code that
% is designed to preserve the operation of \label within \caption
% even when the captionsoff option is in effect. However, because
% of issues like this, it may be the safest practice to put all your
% \label just after \caption rather than within \caption{}.
%
% Reminder: the "draftcls" or "draftclsnofoot", not "draft", class
% option should be used if it is desired that the figures are to be
% displayed while in draft mode.
%
%\begin{figure}[!t]
%\centering
%\includegraphics[width=2.5in]{myfigure}
% where an .eps filename suffix will be assumed under latex, 
% and a .pdf suffix will be assumed for pdflatex; or what has been declared
% via \DeclareGraphicsExtensions.
%\caption{Simulation results for the network.}
%\label{fig_sim}
%\end{figure}

% Note that the IEEE typically puts floats only at the top, even when this
% results in a large percentage of a column being occupied by floats.


% An example of a double column floating figure using two subfigures.
% (The subfig.sty package must be loaded for this to work.)
% The subfigure \label commands are set within each subfloat command,
% and the \label for the overall figure must come after \caption.
% \hfil is used as a separator to get equal spacing.
% Watch out that the combined width of all the subfigures on a 
% line do not exceed the text width or a line break will occur.
%
%\begin{figure*}[!t]
%\centering
%\subfloat[Case I]{\includegraphics[width=2.5in]{box}%
%\label{fig_first_case}}
%\hfil
%\subfloat[Case II]{\includegraphics[width=2.5in]{box}%
%\label{fig_second_case}}
%\caption{Simulation results for the network.}
%\label{fig_sim}
%\end{figure*}
%
% Note that often IEEE papers with subfigures do not employ subfigure
% captions (using the optional argument to \subfloat[]), but instead will
% reference/describe all of them (a), (b), etc., within the main caption.
% Be aware that for subfig.sty to generate the (a), (b), etc., subfigure
% labels, the optional argument to \subfloat must be present. If a
% subcaption is not desired, just leave its contents blank,
% e.g., \subfloat[].


% An example of a floating table. Note that, for IEEE style tables, the
% \caption command should come BEFORE the table and, given that table
% captions serve much like titles, are usually capitalized except for words
% such as a, an, and, as, at, but, by, for, in, nor, of, on, or, the, to
% and up, which are usually not capitalized unless they are the first or
% last word of the caption. Table text will default to \footnotesize as
% the IEEE normally uses this smaller font for tables.
% The \label must come after \caption as always.
%
%\begin{table}[!t]
%% increase table row spacing, adjust to taste
%\renewcommand{\arraystretch}{1.3}
% if using array.sty, it might be a good idea to tweak the value of
% \extrarowheight as needed to properly center the text within the cells
%\caption{An Example of a Table}
%\label{table_example}
%\centering
%% Some packages, such as MDW tools, offer better commands for making tables
%% than the plain LaTeX2e tabular which is used here.
%\begin{tabular}{|c||c|}
%\hline
%One & Two\\
%\hline
%Three & Four\\
%\hline
%\end{tabular}
%\end{table}


% Note that the IEEE does not put floats in the very first column
% - or typically anywhere on the first page for that matter. Also,
% in-text middle ("here") positioning is typically not used, but it
% is allowed and encouraged for Computer Society conferences (but
% not Computer Society journals). Most IEEE journals/conferences use
% top floats exclusively. 
% Note that, LaTeX2e, unlike IEEE journals/conferences, places
% footnotes above bottom floats. This can be corrected via the
% \fnbelowfloat command of the stfloats package.



%\begin{alignat}{1}
%   K(X) = \frac{1}{\sigma {\sqrt {2\,\pi }}} \,e^{-{\frac{(x - \mu)^{2}}{2\sigma^{2}}}}
%\label{eq_AP1:kde_gaussiankernel}
%\end{alignat}


\begin{algorithm}[H]

    \caption{RADAR Signal Simulator}
    \label{DS_simulator} 

    % --------------- Inputs
    \textbf{Inputs}:

    \begin{enumerate}[label={[\arabic*]}, leftmargin = 1cm]
        \item Receptor with the noise level
        \item Emitter Class Database
    \end{enumerate}

    % --------------- Parameters
    \textbf{Parameters}: 
    
    \begin{enumerate}[label = {[\arabic*]}, leftmargin = 1cm]
        \item Number of RADAR present in a signal
        \item Signal size
    \end{enumerate}

    % --------------- Output
    \textbf{Output}: Interlaced labeled signal    
    
\end{algorithm}


\begin{figure}[htbp]
\centerline{\includegraphics[width = 6cm]{/Approach1/DG1_data_final_sub1.png}}
\caption{HDBSCAN temporal clustering result for large cluster 1. Each color identifies a RADAR occurrence.}
\label{fig_AP1:DG1_data_final_sub1}
\end{figure}

Figure~\ref{fig_AP1:DG1_data_final_sub1} shows the result of the temporal clustering performed by HDBSCAN for large cluster 1. The clustering identified each pass of the RADAR. 


\begin{algorithm}[H]
\caption{Decisional Model to prune the dendrogram per branch}
\label{algo_AP1:decisionalmodel} 

\begin{itemize}
    \item Representation of the two first aggregated clusters according to the HACOT by a measure from time of arrival: $\rho$.
    
    \item Application of the Kolmogorov-Smirnov test under the null hypothesis that the two distributions are identical: $\rho_i$ = $\rho_j$

    \begin{description}[font = \normalfont \textitplusparen]
    \item [If: ] $p_{value} > threshold$: 
    
    \begin{itemize}
        \item The 2 clusters are aggregated
        \item Computation of the Kolmogorov-Smirnov test between this aggregated cluster and the next cluster following the branch
        \item Aggregations stop when the top of the tree is reached or when a p-value is not significant
    \end{itemize}
    
    \item [Else: ] $p_{value} \leqslant threshold$ 
    
    \begin{itemize}
        \item The 2 clusters are not aggregated
        \item All groupings above following the branch is no longer considered 
    \end{itemize}
    
    \end{description}
    
    \item Application of the previous steps to the following branches of the dendrogram according to the optimal transport distance.

    \item Repetition until all branches are considered
    
\end{itemize}
\end{algorithm}




\begin{figure}[htbp]
\centerline{\includegraphics[width = 9cm]{/Approach2/data_true_label_full.png}}
\caption{Example of a simulated signal gathering the pulses of four RADARs. Each color identifies a different transmitter.}
\label{fig_AP2:data_true_label}
\end{figure}

%Mettre zoom sur l'étalement ?
%Prendre signal avec 2 cluster bcp plus étalés?
s'affranchir de l'hypothèse de la distribution des clusters le long des lobes



% \textbf{\begin{figure}[h]\centering
% \begin{subfigure}[b]{0.23\textwidth}
%     \centerline{\includegraphics[width = 4cm]{data_description/ot_explanation_deinterlaving.png}}
%     \caption{Example from three simulated distributions.}    \label{fig_DS:ot_explanation_deinterlaving_comment}
% \end{subfigure}%
% \begin{subfigure}[b]{0.23\textwidth}
%     \centerline{\includegraphics[width = 4cm]{Approach1/DG1_ot_explanation_deinterlaving.png}}
%     \caption{Application to clusters 0, 3, and 4.}
%     \label{fig_DS:DG1_ot_explanation_deinterlaving}
% \end{subfigure}
% \caption{Optimal transport functioning between distributions.}
% \label{fig_DS:ot_explanation_deinterlaving_comment}
% \end{figure}}

%In the aggregation strategy, we used an optimal transport distance defined as the cost to move the points from one place to another to quantify this similarity or dissimilarity as highlighted in fig~\ref{fig_DS:ot_explanation_deinterlaving_comment}. The clusters obtained in the plane belonging to the same emitter will have between their distributions a minimal distance.


\begin{figure}[htbp]
\centerline{\includegraphics[width = 8cm]{/data_description/ot_explanation_deinterlaving.png}}
\caption{Time of arrival distribution of 3 simulated distributions. Source and Target 1 distributions 0 and 1 correspond to the same emitter and are active simultaneously, resulting in very few moves to make them match, resulting in low transport cost. Conversely, Source and Target 2 come from 2 different emitters, implying a high transportation cost due to the difference in transmission times.}
%\caption{Time of arrival distribution of 3 clusters. Distributions of clusters 0 and 1 correspond to the same emitter and are active simultaneously, requiring few pulses displacements, so a low transportation cost. Conversely, clusters 0 and 2 come from 2 different emitters, resulting in high transportation cost due to the difference in transmission times.}
\label{fig_DS:ot_explanation_deinterlaving}
\end{figure}


%Fig.~\ref{Chap2_OT_plot:ot_explanations} displays an example of applying optimal transport to define a distance between distributions with identical or disjoint supports. The displacement between the source (in the middle) towards two targets is analyzed. Source and Target 1 have similar appearances resulting in very few moves to coincide Source points toward Target 1 points producing a lower transport cost. Conversely, Source points require significant movement to coincide with Target 2, implying a high transport cost. Optimal transport is utilized to establish a distance; the distance between the Source and Target 1 distribution is set as low, while it will be high between the Source and Target 2 distribution.

%Fig.~\ref{fig_DS:ot_explanation_deinterlaving} illustrates optimal transport on an example of three simulated TOA distributions. Clusters 0 and 1 correspond to different frequencies or pulse widths of the same emitter and are active simultaneously. Consequently, the cost of transporting one TOA distribution to the other is low. Conversely, Clusters 0 and 2 do not belong to the same emitter. Here, pulses sent from cluster 0 to cluster 2 (or reciprocally) must be transported over a considerable distance, implying a higher total transport cost.

%The distributions are dissimilar and are not active simultaneously. Cluster 0 is active four times, whereas cluster 2 is only two at different times. The points in the orange boxes must be sent in multiple directions to be aligned with the red boxes, which have different sizes. A high transport cost will therefore characterize these displacements.
%Conversely, clusters 0 and 1 come from the same RADAR; The two have similar emission patterns. The distribution alignment requires minimal movements. So the transport cost will be defined as the lowest.\\


%In \cite{mottier2021deinterleaving}, fusions were stopped when the optimal transport distance between fused clusters reached a threshold estimated using three unsupervised metrics. However, stopping the fusion at a given optimal transport distance could not handle the variety of possible settings.

%, and the values displayed the associated $p_{value}$ obtained from the Kolmogorov-Smirnov test made from the time of arrival. Pruning a dendrogram is a significant challenge; prematurely stopping the fusions would risk separating several RADARs' pulses into several groups and, lately, stopping grouping them into a single cluster. In a previous article \cite{mottier2021deinterleaving}, we built a decision model using three unsupervised metrics and knowledge of the RADAR environment to set the dendrogram pruning threshold. This method was conclusive when we had low-complexity signals and RADARs with different characteristics. This previous model considered the entire dendrogram to set the pruning threshold and fixed a single threshold following the cluster aggregation order—aggregations made after this threshold was not evaluated. In addition, it could not consider RADARs with similar characteristics. \\

%We propose a new, more efficient version of this decision model based on a simple statistical test to overcome these limitations. The Kolmogorov-Smirnov test\cite{massey1951kolmogorov} and the Student test~\cite{student1908probable} were tested to compare cluster distributions to dendrogram pruning. As a reminder, the Kolmogorov-Smirnov and Student Tests are powerful tests that make it possible to compare two distributions to determine if they come from the same sample under the null hypothesis $H_{0}$. The Kolmogorov-Smirnov test analyzes the difference between the empirical distribution functions of the two samples, and the Student Test compares the averages between two distributions.\\

==> other.tex <==
\begin{figure}[htbp]
\centerline{\includegraphics[width = 9cm]{/data_description/data_unlabeled.png}}
%\caption{Example of a simulated signal gathering the pulses of 4 RADARs. Each color identifies a different transmitter.}
\label{fig_DS:data_unlabeled}
\end{figure}

%\begin{alignat}{1}
%\log L(i |x_{1},x_{2},\dots ,x_{n}) = \sum _{i=1}^{n}\log L(i|x_{i})
   % L(i) = f_{i }(x_{i}) \\
 %  P(X = x_{i} | i ) = \prod _{i=1}^{n}L(i|x_{i}) %\nonumber
%\label{eq_AP1:likelihood}
%\end{alignat}

%We consider that the aggregated clusters obtained following the HACOT contain enough samples to estimate their distribution in a non-parametric way. 
%To estimate their distribution, we use the Kernel Density Estimation. Each aggregated cluster likelihood can be written as: 

with $i$ the aggregated cluster index, $x_1, x_2, ..., x_n$ the cluster pulses, $n$ the number of pulses and $L$ the sample likelihood. We assume that the time of arrival of the pulses is independent:

%\begin{equation} 
%\log L(i |x_{1},x_{2},\dots ,x_{n}) = \sum _{i=1}^{n}\log L(i|x_{i})
  % L(i) = f_{i }(x)   
%\log P(X = x_{i} | i ) = \sum _{i = 1}^{n}\log L(i|x_{i})
%\label{eq_AP1:loglikelihood}
%\end{equation}

==> tools/README <==

August 26, 2015


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.

 2. The \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later.

 3. The \IEEEnoauxwrite command.

 4. The IEEE itemize, enumerate and description list environments.

 5. The complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

 6. The \IEEEQEDhere and \IEEEQEDhereams commands to provide amsthm.sty
    \qedhere functionality to IEEEproof. \IEEEQEDhere is for simple use
    "right on the spot" such as within an IEEEeqnarry:

    \begin{IEEEproof}
       \begin{IEEEeqnarray}{rCl+x*}
        x & = & y & \nonumber\IEEEQEDhere
       \end{IEEEeqnarray}
    \end{IEEEproof}

    While \IEEEQEDhereams is like amsthm's venerable \qedhere and is
    for use within the standard equation environment:

    \begin{IEEEproof}
     \begin{equation}
       x = y \nonumber\IEEEQEDhereams\quad
     \end{equation}
    \end{IEEEproof}

    Note that the qedhere style is normally not done with IEEE-related
    work so these are undocumented features of IEEEtran.cls.

    Thanks Mark D. Butala, Hennadiy Leontyev and Stefan M. Moser for
    suggesting this feature.



IEEEtrantools.sty is not needed and should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
2015/08/26 V1.5 (V1.8b of IEEEtran.cls) changes:

 1) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 2) Fix bug with IEEEeqnarray equation number foreground color
    under the color environment of Beamer class.
    Thanks to Joschi Brauchle for reporting this problem.

 3) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.



********************************** Files **********************************

README                - This file.

changelog.txt         - The revision history.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************


